DistIR: An Intermediate Representation and Simulator for Efficient Neural Network Distribution

The rapidly growing size of deep neural network (DNN) models and datasets has given rise to a variety of distribution strategies such as data, tensor-model, pipeline parallelism, and hybrid combinations thereof. Each of these strategies offers its own trade-offs and exhibits optimal performance across different models and hardware topologies. Selecting the best set of strategies for a given setup is challenging because the search space grows combinatorially, and debugging and testing on clusters is expensive. In this work we propose DistIR, an expressive intermediate representation for distributed DNN computation that is tailored for efficient analyses, such as simulation. This enables automatically identifying the top-performing strategies without having to execute on physical hardware. Unlike prior work, DistIR can naturally express many distribution strategies including pipeline parallelism with arbitrary schedules. Our evaluation on MLP training and GPT-2 inference models demonstrates how DistIR and its simulator enable fast grid searches over complex distribution spaces spanning up to 1000+ configurations, reducing optimization time by an order of magnitude for certain regimes.

==> acknowledgments.tex <==
{\small
\paragraph{Acknowledgments}
Part of the work was done while Keshav was an intern at Microsoft, hosted by Yuan Yu. We thank our shepherd, Sam Ainsworth, as well as Trevor Gale, Fiodar Kazhamiaka, Nuno Lopes, Alberto Magni, Deepak Narayanan, Simon Peyton Jones, Deepti Raghavan, Dennis Shasha, James Thomas, Juliana Vicente Franco, Thomas Wies, and Matei Zaharia for their invaluable feedback. This research was supported in part by affiliate members and other supporters of the Stanford DAWN project---Ant Financial, Facebook, Google, Infosys, NEC, and VMware---as well as Toyota Research Institute, Northrop Grumman, Cisco, SAP, and the NSF under CAREER grant CNS-1651570. Any opinions, findings, and conclusions or recommendations expressed in this material are those of the authors and do not necessarily reflect the views of the National Science Foundation. Toyota Research Institute ("TRI") provided funds to assist the authors with their research but this article solely reflects the opinions and conclusions of its authors and not TRI or any other Toyota entity.}

% We were supported in part by the Stanford DAWN project---including partners Ant Financial, Facebook, Google, Infosys, NEC, and VMware---as well as Toyota Research Institute (``TRI''), Northrop Grumman, Cisco, SAP, and the National Science Foundation (``NSF'') under CAREER grant CNS-1651570. Any opinions, findings, and conclusions or recommendations expressed in this material are those of the authors and do not necessarily reflect the views of the NSF. TRI provided funds to assist the authors with their research but this article solely reflects the opinions and conclusions of its authors and not TRI or any other Toyota entity.


% any ORT folks?, Alberto, Juliana, Nuno, Matei, Keshav's colleagues who gave comments, Dennis, Thomas

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

